Near Data Acceleration with Concurrent Host Access

Near-data accelerators (NDAs) that are integrated with main memory have the potential for significant power and performance benefits. Fully realizing these benefits requires the large available memory capacity to be shared between the host and the NDAs in a way that permits both regular memory access by some applications and accelerating others with an NDA, avoids copying data, enables collaborative processing, and simultaneously offers high performance for both host and NDA. We identify and solve new challenges in this context: mitigating row-locality interference from host to NDAs, reducing read/write-turnaround overhead caused by fine-grain interleaving of host and NDA requests, architecting a memory layout that supports the locality required for NDAs and sophisticated address interleaving for host performance, and supporting both packetized and traditional memory interfaces. We demonstrate our approach in a simulated system that consists of a multi-core CPU and NDA-enabled DDR4 memory modules. We show that our mechanisms enable effective and efficient concurrent access using a set of microbenchmarks, and then demonstrate the potential of the system for the important stochastic variance-reduced gradient (SVRG) algorithm.

==> Makefile <==
PAPER = main
TEX = $(wildcard *.tex)
BIB = $(wildcard bib/*.bib)
FIGS = $(wildcard fig/*.pdf fig/*.png graphs/*.pdf graphs/*.png)
VIEW = open 

all: clean $(PAPER).pdf view

.PHONY: all clean

$(PAPER).pdf: $(TEX) $(BIB) $(FIGS) Makefile
	echo $(FIGS)
	pdflatex $(PAPER)
	bibtex $(PAPER)
	pdflatex $(PAPER)
	pdflatex --synctex=-1 $(PAPER)
	sed -i  -e 's/\/cygdrive\/c/C:/g' $(PAPER).synctex


view:
	$(VIEW) $(PAPER).pdf

clean:
	rm -f *.aux *.bbl *.blg *.log *.out $(PAPER).pdf



==> tex/chonda.tex <==
% !TEX root = ../main.tex

\section{Chopim}
\label{sec:chonda}

In this section, we present a set of solutions to enable concurrent access to the same memory and realize high performance.


\subsection{Opportunistic NDA Issue}
\label{subsec:opportunistic_nda_issue}

The basic policy for Chopim is to aggressively leverage the unutilized rank bandwidth by issuing NDA commands whenever possible. That is, if no incoming host request is detected, NDAs always issue their commands. Since the NDAs can issue whenever there is an opportunity, this maximizes bandwidth utilization. %In addition, since the behavior of NDAs is deterministic, we can still use the replicated FSMs for tracking global state.
One potential problem is that an NDA command issued in one cycle may delay a host command that could have issued in the next. Fortunately, read transactions of NDAs have a small impact on following host commands and ACT and PRE commands are issued infrequently by NDAs. \mdel{However, if an NDA issues a write transaction in one cycle and the next host command is a read, the penalty of write-to-read turnaround is not negligible. We address this below.}

% Even though we can reduce the number of write-to-read interleaving, we cannot entirely avoid this if the NDA operation is write intensive. In such case, the more NDAs issue, the more the host performance is affected. To have a control over the performance of the host and NDAs, we propose the \textit{stochastic NDA issue}. By controlling the probability of NDA issues, we can easily control the performance of the host and NDAs based on priority. To also make this mechanism deterministic, we integrate the same pseudo-random function in both sides so that the sequence of numbers will be random yet the outcomes on both processors will be the same. 

\subsection{Throttling NDA Writes}
\label{subsec:block_nda_write}

%\mattan{a bit repetitive?}
%\benjamin{Sort of. But, unlike above, here I am describing the starvation problem caused by the combination of write-to-read penalty + opportunistic NDA issue.}
When NDAs aggressively issue write commands, the read transactions of the host are blocked due to the penalty for interleaving write-read transactions while write transaction of NDAs keep issuing again since the rank is idle. This degrades host performance while improving NDA performance. To avoid this starvation problem, Chopim provides mechanisms to throttle NDA  write transactions. 

The first mechanism is to issue NDA writes with a predefined probability, reducing the rate of NDA writes. We call this mechanism \textit{stochastic NDA issue}. When NDAs detect rank idleness, they flip a coin and decide whether to issue a write transaction or not. By adjusting the probability, the performance of host and NDAs can be traded off. %Despite the randomness introduced by the stochastic mechanism, the host memory controller can track the NDA issue by integrating the same pseudo-random function. 

The second approach is to predict the rank that the host is going to access next and prevent NDA writes in that rank from issuing. The prediction is based on the requests waiting in the transaction queue. 
% With our baseline FRFCFS scheduler, we observe that the average distance between the queue head and the selected request is less than 1. That is, it is likely that the requests near the queue head will be served next. 
With our baseline FRFCFS scheduler, we observe that the oldest request in the queue will be served next with high likelihood  even though the scheduler can reorder memory operations. In other words, even a simple heuristic can be used to predict the next memory scheduler decision about which rank the host will use. Because the host MC knows whether the NDA that accesses that rank is in write mode or not, it can decide to throttle the NDA.  For the packetized memory interface, such as HMC, no interface change is required to enable this mechanism since one memory controller has all the required information and control over memory requests from both sides. However, for DDR interface, we assume a dedicated pin is available for signaling the NDA to block its next write.

%We add a write buffer in each NDA and push write commands into it instead of issuing right away. When the write buffer overflows, some of data in the write buffer should be written back to memory. In this case, the host memory controller gives an exclusive ownership to the NDA for a short period of time by blocking the host transactions against the rank associated with that NDA. 

% An important decision is that how long should this period be. If it is too long, the access latency of host increases. On the other hand, if this is too short, NDA performance degrades due to bank conflicts; especially, in the small-isolated memory. Let's say there is one NDA bank per rank and NDAs are executing the COPY operation, from $\vec{a}$ to $\vec{b}$. As long as the write buffer is not full, all the memory transactions are for reading $\vec{a}$. However, once it overflows, writing to $\vec{b}$ and reading from $\vec{a}$ will be interleaving. In addition to the write-read turnaround time, the extra bank conflicts occurs because $\vec{a}$ and $\vec{b}$ are in different rows of the same bank. Therefore, these trade-offs should be taken into account when deciding the \textit{exclusive NDA write-back period}. 


% \subsection{Trade-off between Capacity and Performance}
\subsection{Shared vs.~Partitioned NDA/Host Regions}
\label{subsec:tradeoff_cap_perf}

Chopim offers two approaches for utilizing main memory by NDAs. The first is to partition memory such that NDAs only access one subset of memory while regular host loads and stores access the complement subset. Accesses to memory from NDAs and the host are still concurrent. In the second mode, the host and NDAs concurrently access the same range of addresses. The partitioned mode provides isolation and reduces interference. However, partitioning removes physical addresses from the host and assigns them to the NDA. Hence, changing partitioning decisions should be done infrequently, reducing flexibility. \madd{On the other hand,} Sharing provides flexibility in which data is processed by the NDA and eliminates the need for data copies. The two modes can be mixed with a portion of memory dedicated to NDA access and other regions that are shared, though we do not explore mixed isolation and sharing in this paper.
%Chopim uses a new bank partitioning interface and mechanism for isolation and a common data layout for shared regions, as described below.

We address two main challenges to enable the two modes above. 
The challenge with sharing addresses between host and NDAs is in how data is laid out across memory locations. The typical layout for the host spreads data across DRAM chips and ranks, but chip- and rank-locality is required for the NDAs. We resolve this data alignment issue by rearranging data at the host memory controller for chip-locality and relying on physical frame contiguity or page coloring by the OS. %extending the bank partitioning mechanism to place data in a specific group of rows for rank-locality. At the same time, the OS ensures that memory allocation is aligned with this coarser granularity. We discuss the details in \sect{subsec:impl_data_layout}. We confirm that this does not degrade host memory bandwidth utilization and do not observe any measurable impact on host performance in our simulations.
We use \textit{bank partitioning} to provide isolation and minimally impact host performance. We develop a new bank partitioning mechanism that permits the use of sophisticated physical-to-DRAM address mapping functions, \madd{even when huge pages that span many banks are used}. 
%We require the OS to reserve a region at the top of its physical memory address range and notify hardware of how much memory is dedicated to the NDAs. The memory controllers then map these addresses to a subset of the banks while still distributing host addresses across the remaining banks. Our approach  works with any page size and flexible address mapping, and we can partition banks arbitrarily. We discuss our implementation in detail in \sect{subsec:impl_bpart}. 
%\textbf{Shared Data Layout.}


% \subsection{Data Alignment in Large-shared Memory}
% \label{subsec:impl_page_color}

% Unlike the small-isolated memory region, address mapping cannot be optimized, such as skipping address hashing, for NDAs in the large-shared region. Therefore, to enable NDA and concurrent access in this region, data should be carefully laid out considering the address hashing of the host memory controller and locality for NDAs. 

% The address hashing shuffles data across channels, ranks, and banks. To layout data such that elements with same index are located in the same rank, hashing for channel and rank bits should be prevented or should be done with the same key. To maintain the original host address mapping, we choose the latter approach and can be done with page coloring. For the operands within one process, the LSBs of row address that are used for hashing channel and rank bits should be colored with the same value. For the huge page, OS cannot control the key for channel bits. We use the same remapping scheme that is used in bank partitioning. 

% Only with page coloring does not guarantee the desired data layout. In addition to the page coloring, OS should help aligning the base address of operands and align other elements as well. We use buddy allocator [?] and always allocate memory for NDA operands in the granularity of rows in the system, e.g. all the row \texttt{0}s in the system. If we force the buddy allocator to allocate contiguous memory in a coarse granularity, the base addresses of operands will be naturally aligned. For the same reason, using huge page can also be an alternative solution. 



% \textbf{Shared Data Layout.}
% The challenge with sharing addresses between host and NDAs is in how data is laid out across memory locations. The typical layout for the host spreads data across DRAM chips and ranks, but chip- and rank-locality is required for the NDAs. We resolve this data alignment issue by rearranging data at the host memory controller for chip-locality and extending the bank partitioning mechanism to place data in a specific group of rows for rank-locality. At the same time, the OS ensures that memory allocation is aligned with this coarser granularity. We discuss the details in \sect{subsec:impl_data_layout}. We confirm that this does not degrade host memory bandwidth utilization and do not observe any measurable impact on host performance in our simulations.

\mcut{Our simulation results  
The second memory option is the large-shared memory where the host and NDA transactions contend for the same banks. As a result, extra bank conflicts occur while interleaving transactions and this significantly degrades NDA performance. On the other hand, NDAs can be used without worrying about the capacity limit in this large-shared memory region. However, to allow concurrent access to the same data in this region, a data alignment issue should be resolved.
% In the large-shared memory, the baseline address mapping is used and its address hashing causes a data alignment issue for NDAs. Typically, the address hashing is used for shuffling data across the banks in the system to minimize the number of bank conflicts. On the other hand, in the perspective of NDAs, to avoid data movement between NDAs, operands should be aligned such that the elements with the same index are located in the same rank. However, the address hashing messes up the data alignment required for NDA operations. 
In the large-shared memory, the baseline address mapping is used and its address hashing causes a data alignment issue for NDAs. Typically, address hashing is used to shuffle data across banks in the system but this hinders localizing operands of NDA operations.
\mattan{To here. Too long to make point.} \benjamin{Done.} To solve this problem, we apply the same page coloring and remapping mechanism in a slightly different way. The detailed mechanism is explained in Section \ref{subsec:impl_data_layout}.
}

% \benjamin{I made the following two sections as the subsection of this one.}

% \subsection{Data Alignment in Large-shared Memory}
% \label{subsec:impl_page_color}

% Unlike the small-isolated memory region, address mapping cannot be optimized, such as skipping address hashing, for NDAs in the large-shared region. Therefore, to enable NDA and concurrent access in this region, data should be carefully laid out considering the address hashing of the host memory controller and locality for NDAs. 

% The address hashing shuffles data across channels, ranks, and banks. To layout data such that elements with same index are located in the same rank, hashing for channel and rank bits should be prevented or should be done with the same key. To maintain the original host address mapping, we choose the latter approach and can be done with page coloring. For the operands within one process, the LSBs of row address that are used for hashing channel and rank bits should be colored with the same value. For the huge page, OS cannot control the key for channel bits. We use the same remapping scheme that is used in bank partitioning. 

% Only with page coloring does not guarantee the desired data layout. In addition to the page coloring, OS should help aligning the base address of operands and align other elements as well. We use buddy allocator [?] and always allocate memory for NDA operands in the granularity of rows in the system, e.g. all the row \texttt{0}s in the system. If we force the buddy allocator to allocate contiguous memory in a coarse granularity, the base addresses of operands will be naturally aligned. For the same reason, using huge page can also be an alternative solution. 


\subsubsection{Data Layout for Shared Addresses}
\label{subsec:impl_data_layout}

% While bank partitioning provides isolation, it prohibits close cooperation of both the host and NDAs processing the same data in the same memory.
Data layout in a shared region is challenging because the host and NDAs have different constraints or preferences for data layout: the host prefers spreading addresses across chips, ranks, banks, and channels to maximize bandwidth and reduce bank conflict likelihood while the NDAs require contiguity within chips and ranks. To satisfy both, we focus on laying out data at the chip (device) and rank levels. 
% Unlike the partitioned memory region, address mapping cannot be optimized, such as skipping address hashing, for NDAs in the shared region. Therefore, to enable concurrent access in this region, data should be carefully laid out considering the address hashing of the host memory controller and locality for NDAs. To satisfy both requirements, we focus on the data layouts at two levels of memory hierarchy: device and rank levels.

% As briefly discussed in Section \ref{subsec:impl_bpart}, data should be laid out such that all the operands are placed in local memory to avoid communication among NDAs. On the other hand, data layout for the host processor is usually spread out across memory channels, ranks, and banks to exploit memory-level parallelism. To satisfy both requirements in the large-shared memory region, we focus on the data layouts at two levels of memory hierarchy: device and rank levels. 

\medskip
\noindent\textbf{\textit{Data Layout Across DRAM Chips.}}
In the baseline system, each \rev{4-byte} word is striped across multiple chips, % (\fig{fig:baseline_chip_layout}),
whereas in our approach each word is located in a single chip so that NDAs can access words from their local memory. %(\fig{fig:proposed_chip_layout}).
Both the host and NDAs can access memory without copying or reformatting data (as required by prior work~\cite{farmahini2015nda}). Memory blocks still align with cache lines, so this layout change is not visible to software. This layout precludes the critical word first optimization from DRAM, but recent work concludes the impact is minimal because the relative latency difference in current memory systems is very small (e.g.,~\cite{yoon2012dgms}). 

% \begin{figure}[t!]
% \centering
% 	\subfloat [Baseline] {
% 		\includegraphics[width=0.46\textwidth]{fig/baseline_chip_layout.pdf}
% 		\label{fig:baseline_chip_layout}
% 	}\\
% 	\subfloat [Proposed] {
% 		\includegraphics[width=0.46\textwidth]{fig/proposed_chip_layout.pdf}
% 		\label{fig:proposed_chip_layout}
% 	}\\
% 	\caption{On-the-fly rearrangement for concurrent access. In this example, we assume the DIMM has four x8 chips with prefetch depth 4. The size of each data block is 1 byte.}
% 	\label{fig:chip_layouts}
% \end{figure}

\medskip
\noindent\textbf{\textit{Data Layout Across Ranks.}}
A typical physical to DRAM address hash-based mapping rearranges contiguous addresses across multiple DRAM ranks and banks, breaking the locality needed for NDAs. \fig{fig:rank_layout} shows an example of naive data layout by using the baseline address mapping (left) and the desired layout for shared regions (right). \madd{In the naive layout}, the first element of vector ${A}$ and that of vector ${B}$ are located in different ranks, breaking NDA locality. That same data is in the same rank in the desired layout, while still satisfying host access requirements \madd{for high bandwidth and low bank contention}. We achieve the desired behavior by mapping NDA operands that are used together to groups of frames that all have the same \sout{shuffling} \rev{interleaving} pattern across channels and ranks. In this way, as long as their initial column alignment is the same, all operands remain aligned even though elements are spread across banks and ranks.

% Sentences below basically repeat last sentence above.
%\badd{To implement this mechanism, two requirements should be met when the runtime system allocates frames for NDA operands. First, the base addresses of operands should be aligned such that their column addresses are the same. Second, when the rank switches as the index to elements increases, all operands should switch to the same rank so that the elements of operands with the same index still are located in the local rank.}

\madd{Our current implementation achieves this using coarse-grain memory allocation and coloring. 
We allocate memory such that operands are aligned at the granularity of one DRAM row for each bank in the system which we call a \textit{system row} (e.g., 2MB for a DDR4 1TB system). This is simple with the common buddy allocator if allocation granularity is also a system row, and can use optimizations that already exist for huge pages~\cite{yun2014palloc,kwon2016coordinated,gorman2004understanding}. The fragmentation overheads of coarse allocation are negligible because there is little point in attempting NDA execution for small operands.}

\madd{In our baseline address mapping~\ref{fig:baseline_addr_map}, the rank and channel addresses are determined partly by the low-order bits that fall into the frame offset field and partly by the high-order bits that fall into the physical frame number (PFN) field. The frame offsets of operands are kept the same because of the above alignment. On the other hand, PFNs are determined by the OS. Therefore, to keep those high-order bits the same among operands, the Chopim runtime indicates a \textit{shared color} when it requests memory from the OS and uses the same color for all operands of a specific NDA operation. The OS uses the color information to ensure that all operands with the same color (same shared region) follow the same channel and rank interleaving pattern. To do this, the OS needs to know which physical address bits are used to select ranks and channels by the host memory controller. Coloring limits the region size because the bits that determine rank and channel must have the same value within the region. Multiple regions can be allocated for the same process. \rev{Though we focus on one address mapping here, we believe our approach of coarse-grain and address-mapping-aware allocation can be generalized and applied to other address mappings as well.}}

% \benjamin{Rewrote from here...}
% To implement this mechanism, two conditions should be satisfied when the runtime system allocates frames for NDA operands. First, the base addresses of operands should be aligned such that the frame offset fields are the same. \mattan{offsets of what are the same? All operands touched by NDA? All operands touched by particular kernel? ... Be explicit in the previous sentence.} Then, the low-order bits are the same among operands. Our runtime system allocates memory at a coarse granularity such that each operand spans all address bits used to determine column, bank, rank, and channel addresses to ensure initial alignment. This is the granularity of one DRAM row for each bank in the system (e.g., 4MB for a DDR4 2TB system), which we call a \textit{system row}. Note that the OS should guarantee that this coarse-grain memory region is contiguous in the physical memory space. \mattan{Is this a bit pessimistic? Could it be that some other granularity can still guarantee it with appropriate coloring? Maybe not, I didn't think about this enough (or at all).}

% Next, the allocated frames for the operands should correspond to system rows that have the same shuffling pattern across channels and ranks. Typically, the shuffling pattern is partly determined by the high-order bits that fall into the physical frame number (PFN) allocated by the OS. Therefore, we use an OS-controlled page coloring approach to make those high-order bits the same among the operands. This mechanism requires the OS to know which physical address bits are used to select ranks and channels by the host memory controller. When the runtime memory allocator requests memory from the OS, it indicates that it should be shared with the host and assigns it a specific \emph{shared color}. The OS uses the color information to ensure that all operands within the same shared region (same color) follow the same channel and rank interleaving pattern, and thus remain aligned. \mattan{I assume you sort of implemented this? If so, state that you did. Maybe add appendix with ``algorithm'' for this?}
% \benjamin{To here...}

% \madd{There are two options for grouping frames to follow the same hashing pattern. The first is to use coarse-grain physical memory allocation for NDA operands such that each operand spans all address bits used to determine bank, rank, and channel address. This is the granularity of one DRAM row for each bank in the system, which typically is less than 2MB. Thus, as long as operands are aligned to 2MB huge pages, their hashing pattern will be the same.} \mattan{I don't understand the text below. Good chance it's because I'm falling asleep. However, would be good if we discuss or if Benjamin tries a rewrite. I'm not sure which bits get colored here and I'm not sure what the alignment granularity is at the end.}

% We use an OS-controlled page coloring approach that, unlike bank partitioning, does require knowledge of which physical address bits are used to select ranks and channels. First, when the runtime memory allocator requests memory from the OS, it indicates that it should be shared with the host and assigns it a specific \emph{shared color}. Second, the runtime system allocates memory to NDA operands with virtual addresses that are aligned to either huge pages or, if larger than 2MB, the size of one DRAM row across every bank in the system (e.g., 4MB for a DDR4 2TB system). Third, the OS uses the color information to ensure that all operands within the same shared region (same color) follow the same channel and rank interleaving pattern, and thus remain aligned. Within a shared region, the OS allocates physical frames that are contiguous and aligned to the same granularity the runtime allocator uses. This implies that all address bits within the alignment granularity mentioned above are inherently aligned between operands as all operand origins are aligned. Hence, the OS simply assigns the same values to all higher-order bits that affect channel and rank to all frames within a region to ensure the desired behavior. 


% \benjamin{To support a unified layout for huge page, the similar approach is used for bank partitioning, such as collaboration between OS and memory controller. The difference is that the OS needs to know the address hash function of the host memory controller. The OS colors one of the row bits (with green) that is used as the key to determine the rank bit in \fig{fig:huge_page_coloring}. Next, we determine one row bit that is used for remapping and, in our design, we use the next MSB bit (left red bit) after the ones that are reserved for bank partitioning. Then, when the memory controller translate physical-to-DRAM address, this bit is compared with the bit that is used for determining the channel bit (right red bit). If those are the same, we stick with the original address mapping. Otherwise, we swap the bits between two red bits. This allows remapping rows such that the same address shuffling pattern is used within 2MB page (\fig{fig:huge_page_remapping}).}

% \begin{figure}[t!]
% \centering
%   \subfloat [Huge page coloring.] {
% 		\includegraphics[width=0.46\textwidth]{fig/huge_page_coloring.pdf}
% 		\label{fig:huge_page_coloring}
% 	}\\
% 	\subfloat [Huge page remapping.] {
% 		\includegraphics[width=0.4\textwidth]{fig/huge_page_remapping.pdf}
% 		\label{fig:huge_page_remapping}
% 	}\\
% 	% \includegraphics[width=0.48\textwidth]{fig/huge_page_coloring.pdf}
% 	\caption{Page coloring and remapping for huge page to provide unified address mapping.}
% 	\label{fig:huge_page_coloring}
% \end{figure}


% Sim
% To maintain the original host address mapping and solve the alignment issue, we use page coloring with remapping in a slightly different way than our bank partitioning. For the address of operands that belong to the same process, the LSBs of row address that are used for hashing channel and rank bits should be colored with the same value. For huge page support, OS cannot control the key for channel bits. Therefore, we use the same remapping scheme that is used in bank partitioning.

% In addition, to put the elements of operands with the same index together in the same rank, we align the first element and allocate contiguous memory to align other elements as well. 

% Only with page coloring does not guarantee the desired data layout. In addition to the page coloring, OS should help aligning the base address of operands and align other elements as well. We use buddy allocator and always allocate memory for NDA operands in the granularity of rows in the system, e.g. all the row \texttt{0}s in the system. If we force the buddy allocator to allocate contiguous memory in a coarse granularity, the base addresses of operands will be naturally aligned. For the same reason, using huge page can also be an alternative solution. 

% \begin{figure*}[t!]
% \centering
% 	\includegraphics[width=0.65\textwidth]{fig/rank_layout.pdf}
% 	\caption{Data alignment for concurrent access. For brevity, we depict only 4 banks per rank. Each data block represents interleaving granularity, which is 128 bytes in our baseline.}
% 	\label{fig:rank_layout}
% 	\vspace*{-4mm}
% \end{figure*}

\begin{figure*}[t!]
	\centering
	\begin{minipage}[t]{0.95\textwidth}
		\begin{minipage}[t]{0.6\textwidth}
			% \vspace*{4mm}
			\subfloat [Data layout across ranks for concurrent access.] {
				\includegraphics[width=\textwidth]{fig/rank_layout.pdf}
				\label{fig:rank_layout}
			}
		\end{minipage} %
		\quad %
		\begin{minipage}[t]{0.4\textwidth}
			\subfloat [Baseline address mapping] {
				\includegraphics[width=\textwidth]{../fig/baseline_addr_map.pdf}
				\label{fig:baseline_addr_map}
			} \\
			\subfloat [Host-side address mapping for bank partitioning.] {
				\includegraphics[width=\textwidth]{../fig/hashing_addr_map.pdf}
				\label{fig:hashing_addr_map}
			}
		\end{minipage}
	\end{minipage}
	\caption{Data layout (shared region) and bank partitioning (partitioned region).}
	\label{fig:addr_map}
	% \vspace*{-3mm}
\end{figure*}

\subsubsection{Bank Partitioning}
\label{subsec:impl_bpart}

Prior work on bank partitioning relies on the OS to understand how physical addresses are mapped to banks~\cite{mi2010bankpark,jeong2012balancing,liu2012software}. The OS colors pages to assign them to different bank partitions and then allocate frames that map to a specific set of banks to a specific set of colors. Memory accesses for different colors are then isolated to different banks. Colors can be assigned to different cores or threads, or in our case, for host and NDA isolated use. Unfortunately, advanced physical-to-DRAM address mapping functions and the use of 2MB pages prevent prior bank partitioning schemes from working because the physical frame number (PFN) bits that the OS can control can no longer specify arbitrary bank partitions. 

\fig{fig:baseline_addr_map} shows an example of a modern physical address to DRAM address mapping \cite{pessl2016drama}. One color bit in the baseline mapping belongs to the page offset field so bank partitioning can, at best, be done at two-bank granularity. More importantly, when huge pages are used (e.g., 2MB), this baseline mapping cannot be used to partition banks at all. 

To overcome this limitation, we propose a new interface that partitions banks into two groups---host- and NDA-reserved banks---with flexible DRAM address mapping and any page size. Specifically, our mechanism only requires that the most significant physical address bits are only used to determine DRAM row address, as is common in recent hash mapping functions, as shown in \fig{fig:hashing_addr_map}.

Without loss of generality, assume 2 banks out of 16 banks are reserved for the NDA. First, the OS splits the physical address space for host and NDA with the host occupying the bottom of the address space: $0-\left(14\times\mathit{(bank\_capacity)}-1\right)$. The rest of the space (with the capacity of 2 banks) is reserved for the NDA and the OS does not use it for other purposes. This guarantees that the most significant bits (MSBs) of the host address are never b'111. In contrast, addresses in the NDA space always have b'111 in their MSBs. % (bank b'1111 and b'1110).

The OS informs the memory controller that it reserved 2 banks (the topmost banks) for NDAs. Host memory addresses are mapped to DRAM locations using any hardware mapping function, which is not exposed to software and the OS. The idea is then to remap addresses that initially fall into NDA banks into the reserved address space that the host is not using. Additional simple logic checks whether the resulting DRAM address bank ID of the initial mapping is an NDA reserved bank. If they are not, the DRAM address is used as is. If the DRAM address is initially mapped to a reserved bank, the MSBs and the bank bits are swapped. Because the MSBs of a host address are never b'1110 or b'1111, the final bank ID will be one of the host bank IDs. Also, because the bank ID of the initial mapping result is 14 or 15, the final address is in a row the host cannot access with the initial mapping and there is no aliasing. %Basically, this mechanism remaps the addresses that originally belong to the NDA banks to the reserved address space that belongs to the host banks.
%\todo[inline]{Mattan doesn't understand why the mechanism above is guaranteed to work with any hashing scheme. How do you prove that? Maybe if MSBs only used to determine row with the original hash?}

\medskip
\noindent\textbf{\textit{Host Access to NDA Region.}}
The OS does not allocate regular host addresses in the NDA region, but some host requests will read and write NDA data to provide initial inputs to NDA operations and read outputs. Requests with addresses that map to the NDA region use a mapping function that does not hash bank addresses and simply uses the address MSBs for banks. This ensures that NDA addresses only access NDA-reserved banks. Furthermore, the way other address bits are mapped to DRAM addresses is kept simple and exposed to software. 

% , the memory controller To allow the host to access NDA data, a special interface is required to allocate and access the memory space of NDAs. If the memory is allocated with a special API call, say ${nda\_malloc()}$, memory will be allocated and mapped to the physical address of which MSBs are b'1111 (15). These bits are used to specify the bank ID. For element-wise operations, the elements with same index of operands should be placed in the same rank to avoid any NDA-to-NDA communication. However, the address mappings that adopt hashing, such as the ones in \ref{fig:addr_map}, shuffles the contiguous address space across channels and ranks, which makes it hard to align operands. To avoid the problem, no hashing is used for the address space of NDAs. Therefore, once the address of request has b'1111 in its MSBs, the memory controller uses a different address mapping than the one used for normal memory access. In this way, the host can access the NDA data and NDAs can keep all the operands in their local memory. 

% \begin{figure}[t!]
% \centering
% 	\subfloat [Baseline] {
% 		\includegraphics[width=0.46\textwidth]{../fig/baseline_addr_map.pdf}
% 		\label{fig:baseline_addr_map}
% 	}\\
% 	\vspace*{-4mm}
% 	\subfloat [Host-side address mapping for bank partitioning] {
% 		\includegraphics[width=0.46\textwidth]{../fig/hashing_addr_map.pdf}
% 		\label{fig:hashing_addr_map}
% 	}\\
% 	\caption{Baseline and proposed address mapping.}
% 	\label{fig:addr_map}
% 	\vspace*{-2mm}
% \end{figure}

\subsection{Tracking Global Memory Controller State}
\label{subsec:track_gstate}

Unlike conventional systems, Chopim also enables an architecture that has two memory controllers (MCs) managing the bank and timing state of each rank. \madd{This is the case when the host continues to directly manage memory even when the memory itself is enhanced with NDAs}, which requires coordinating rank state information. Information about host transactions is easily obtained by the NDA MCs as they can monitor incoming transactions and update the state tables accordingly. However, the host MC cannot track NDA transactions due to command bandwidth limits. 

To solve this problem, we leverage the deterministic execution flow of the NDA workloads that we focus on. Once the base address of operands and the operation type are determined, NDAs access memory deterministically and are controlled by microcode and a finite state machine (FSM). If the FSMs are replicated and located also in the host side, the host MC effectively tracks all NDA transactions. Also, the host MC knows its next transaction and target rank. With this information, the host MC deduces which NDA will be affected by its transactions and for how long. Thus, the host MC can track the global state in real time without any communication. \madd{Stochastic NDA issue is still easily supported by replicating the pseudo-random number generator.}
%\mattan{Any problems with refresh or are we assuming that's host-managed as well? Makes sense to me that still host managed and we don't need to say anything, but want to confirm.} \benjamin{I actually enabled memory refresh in the simulation and I confirm that there is no problem. The host memory controller manages it.}

% \benjamin{Added one paragraph, one figure, and one discussion.}
% \mattan{This is still confusing. Specifically, I think ``updated accordingly'' is confusing -- how is that done? What signal/command? Or is it implicit? It might be that I'm only confused because I'm editing now and not really reading like a reader.}
% \benjamin{Clarified.}
Figure \ref{fig:repl_fsm} shows example operations of the replicated FSMs where one rank is being accessed by the host (left) and the other by an NDA (right). When the host accesses rank0, both host and NDA memory controller state is updated based on the issued host command. On the other hand, when the host does not access but NDA1 accesses rank1 (right), the host-side replicated FSM updates its state of rank1 in the host memory controller. This mechanism is not required when only a single memory controller exists for each rank, as with a packetized memory interface~\cite{pawlowski2011hybrid,genz2017genz,kim2013memory}.

\medskip
\noindent\textbf{\textit{Discussion.}} \madd{A current limitation of our replicated-FSM approach is that it applies to workloads with generally data-independent behavior \rev{where execution flow is not determined by data values}. This includes a rich and important set of applications and kernels that are of practical importance. We leave extensions to more data-dependent workload behavior to future work. We also note that the particular synchronization problem does not exist in a packetized memory interface, while the other problems we address still do. We consider this work a starting point on illuminating and solving a set of problems for NDAs that share their physical memory with the host and where applications tightly collaborate across the host and NDAs.}
%  As other accelerators, such as GPUs, were developed to target specific applications at the beginning and then has evolved later to accommodate diverse applications, we envision that the combination of the host and NDAs can accelerate many different applications in the future. However, instead of trying to accelerate many types of workloads in this paper, we focus on what needs to be done to support concurrent access from the host and NDAs to the same memory. 

\begin{figure}[t!]
\centering
        \includegraphics[width=0.37\textwidth]{fig/repl_fsm.pdf}
	\caption{Example operation of replicated FSMs.}
	\label{fig:repl_fsm}
	% \vspace*{-4mm}
\end{figure}


% \subsection{Exploiting Locality across NDA Operations}
% \label{subsec:locality_scratchpad}
% We leverage data reuse opportunities across NDA operations to reduce NDA memory transactions. One example workload that exploits locality is element-wise averaging. During averaging, the intermediate sum is stored in one vector and is continuously reused for accumulation. In this case, instead of writing the intermediate sum to DRAM, Chopim introduce a scratchpad memory to reduce the number of write transactions.\mattan{This isn't clear. Why are there intermediate if constantly updating the same vector?} The size of scratchpad memory per rank is 8KB, which is equivalent to the size of the DRAM row buffer across the rank. If the size of each vector is larger than 8KB, the operation is stripmined. %NDAs average for first 8KB of the vectors, write the result to DRAM, and move on to the next chunk. 

% \subsection{Mitigating Load Imbalance} \mattan{can't parse these}\benjamin{Edited.}
% \label{subsec:short_iter_nda}
% Some NDA operations use relatively short vectors and multiple iterations. 
% In applications using vector operations, there are cases that each operation is rather short but executed iteratively. Compared to one long NDA operation, these short-living operations suffer from load imbalance. 

% % \noindent\textbf{\textit{Mitigating Workload Imbalance.}}
% Within a wide range of time, all the ranks in the systems are evenly accessed by the host. However, within a short time range, the host tends to access several ranks more than others. This short-term access pattern of the host results in workload imbalance of NDAs, especially when each NDA operation takes short time. To solve this imbalance problem, Chopim supports \textit{asynchronous launching} when possible, instead of waiting until all the NDAs finish their previous operations. This mechanism enables NDAs to offset the short-term imbalance over the iterative NDA execution. However, when an operation requires reduction across NDAs, such as dot product, this mechanism cannot be used. % Note that this asynchronous launching cannot be used after dot product when the following NDA operation consumes the result of dot product since the final reduction is required. 

% \todo[inline]{Not clear at all. Kind of long and not clear what async means or implies}\benjamin{Tried to clarify.}


% \todo[inline]{Rewrite. Readers has no idea what this is about. It's not discussed in "workloads", so much better description needed here.}\benjamin{Rewrote.}
 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tex/motivation.tex <==
% !TEX root = ../main.tex

\section{Opportunities and Challenges}
\label{sec:motivation}

In multi-programmed systems, NDA-integrated memory devices will be main memory for some processes and accelerators for other processes. Furthermore, the host and NDAs should access the same memory in parallel when collaboratively processing data. Under this scenario, it is necessary to effectively share memory between the host and NDAs. In this section, we identify opportunities to better utilize internal rank bandwidth compared to prior approaches and discuss four problems that we solve to utilize that bandwidth.

\subsection{Prior Approaches}
\label{subsec:prior_work}

Prior work \cite{farmahini2015nda} proposes two ways to share memory between the host and NDAs. First, the ownership of each rank is ping-ponged between the host and NDAs in a coarse-grain manner. Before ownership is exchanged, all the banks are precharged so that the next owner can start accessing memory from the initialized state. Since warming up memory takes time, ownership transitioning should be done in coarse granularity to amortize this overhead. However, coarse-grain ownership switching results in halving the performance of both owners compared to their ideal performance. 

The second way is to partition ranks into two groups with each processor having exclusive ownership over one group of ranks. This approach eliminates the source of contention and ownership switching overhead. However, a large portion of memory capacity should be assigned to NDAs and the potential bandwidth gain of NDAs is limited by the number of ranks dedicated to NDAs. 

\subsection{Opportunity: Rank Idle Periods}
\label{subsec:opportunities}
Because multiple ranks share the command and data buses within each channel, the host can access only one rank at a time per channel. In addition, to avoid rank switching penalty, memory controllers tend to minimize rank interleaving. As a result, ranks are often not accessed by the host for certain periods of time. \fig{fig:motiv_rank_idle} shows the bandwidth utilization of rank internal buses when only host programs are executed. Our application mixes and the baseline configuration are summarized in Table \ref{tab:eval_config}. Overall, about 60\% of the internal-bus bandwidth is unused. However, the majority of idle periods are just $10-250$ cycles. 

By opportunistically issuing NDA memory commands in these idle periods, we can better utilize internal rank bandwidth. Compared to the prior approaches, \textit{fine-grain interleaving of NDA access minimally impacts the performance and memory capacity of the host while maximizes the utilization of rank bandwidth}. 

\begin{figure}[t!]
\centering
	\includegraphics[width=0.48\textwidth]{fig/motiv_rank_idle.pdf}
	\caption{Rank idle-time breakdown vs. idleness granularity.}
	\label{fig:motiv_rank_idle}
	\vspace*{-4mm}
\end{figure}

\subsection{Challenge 1: Fine-Grained Access Interleaving}
\label{subsec:challenges}
To opportunistically issue NDA commands, mechanisms for fine-grain mode switching are required, raising the following challenges. 

\medskip
\noindent\textbf{\textit{Extra Bank Conflicts.}}
Since the host and NDAs share banks, fine-grain access interleaving is likely to cause additional bank conflicts. Opening and closing rows incur overhead and hinder utilizing rank bandwidth within short idle periods. 
%Especially, our NDA workloads have streaming access pattern and it can maximally benefit from row buffer hits. However, even a few extra bank conflicts can significantly degrade NDA performance. 

\medskip
\noindent\textbf{\textit{Read/Write Turnaround Time.}}
As discussed in Section \ref{sec:background}, interleaving read and write operations to the same rank incurs extra overhead compared to issuing the same command type back to back \cite{stuecheli2010virtual}. The host mitigates this overhead by buffering operations with caches and write buffers. However, without coordination, the host and NDAs may issue different types of transactions, which are then interleaved if both host and NDA run in parallel. Therefore, we need a mechanism to throttle write transactions of NDAs when needed and allow issuing when the rank is idle for long enough time. 
% However, a naive approach to concurrent access may cause interleaving between NDA's write and host's read transactions. We can also add write buffers to NDAs but write-intensive NDA workloads require large write buffer, which incurs area and power overhead. Therefore, at some point, there will be many interleaving and it needs to be handled appropriately. 

%\benjamin{Moved to the end of this subsection and specified that this challenge is only for DIMM-type DRAM devices.}
\medskip
\noindent\textbf{\textit{Overhead of State Coordination.}}
For DIMM-type DRAM devices, each NDA needs its own memory controller to allow NDAs to utilize the untapped bandwidth. This results in two memory controllers managing the bank and timing state of each rank. To synchronize the state between the two memory controllers, prior work adopts the precharge-all (PREA) mechanism. However, fine-grain mode switching will incur significant overhead not only because of PREA command overhead itself but also because of the warm-up time required after mode switching. 


% \noindent\textbf{\textit{Data Layout and Address Mapping.}}
\medskip
\subsection{Challenge 2: Unified Data Layout for Collaboration}
% \benjamin{I made this as a separate subsection.}
When either just the host or just the NDAs own a rank for a fairly long time, we can customize data layout and address mapping for each processor, possibly copying and laying out data differently when switching access modes. However, concurrent NDA and host access to the same data requires a single data layout and address mapping that works well for both the host and NDA at the same time. Otherwise, two copies of data with different layouts are necessary, incurring high capacity overhead. 

%\todo[inline]{These challenges should appear in intro (possibly abstract too).}\benjamin{Added to intro. Will add to abstract as well.}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tex/motivation2.tex <==
% !TEX root = ../main.tex

\section{Motivation}
\label{sec:motiv}
We motivate our work with three key questions for a main-memory NDA, which we later answer with the Chopim architecture.
%In this section, we explain the three main questions that we address. The first question is about the case where the host and NDAs access different data but still share the same memory devices. On the other hand, the second question asks about how to deal the situation where the host and NDAs share the same data and access them concurrently. The third question is about how the above questions can be answered under direct host control on non-packetized DRAMs.

\medskip
\noindent\textbf{\textit{Q1: How can NDA-enabled DRAM be simultaneously used for both compute and host high-capacity memory?}} 
% - Should the host and NDAs time-share memory devices? (with periodical mode switching)
% - How to mitigate overheads for switching access points? (write-to-read penalty, global state management, bank conflicts)

As NDA-equipped memory devices are not only accelerators but also main memory, it is important to effectively manage the situation where memory is simultaneously accessed by both the host and NDAs. \textit{The main challenge is how to maximize NDA performance and minimize host performance degradation while avoiding conflicts on the shared data path between the host and NDAs.} % For instance, if one application accesses the memory devices that are currently being accessed internally by NDAs to accelerate another application, it is unclear how to manage them and which one should be prioritized over the other. 
Prior work solves this in three directions: \textit{unified memory interface}, \textit{spatial partitioning}, and \textit{time sharing}. In the first approach, every memory requests for the host and NDAs are managed in one place and issued through the same memory interface. However, as all the memory commands are transferred through the same bus, performance scalability along with the number of ranks is limited by the command-bus bandwidth. The next two approaches solve this by separating the memory interface of the host and NDAs. We also assume that each NDA can independently access memory with its own MC.

The second approach partitions memory into two independent groups (e.g. group of ranks) and allows the host and NDAs to exclusively access their own group of memory [?]. This approach requires a large fraction of memory capacity to be reserved for NDAs. Moreover, the potential bandwidth gain of NDAs is limited by the number of ranks dedicated to NDAs. In time-sharing, ownership of memory alternates between the host and NDAs and only one of them accesses memory [?]. Before the ownership switches, an existing mechanism initializes all the bank state which incurs overhead due to the initialization and warm-up overhead. Therefore, coarse-grain switching is required to amortize the overhead (see Section ? for more details). However, in this mechanism, how much time is allocated for each processor determines performance of the host and NDAs. 

To mitigate this strict performance tradeoff, our approach leverages the internal memory bandwidth for NDA execution that are unutilized while the host accesses memory. \fig{fig:motiv_rank_idle} shows the bandwidth utilization of rank internal buses when only memory-intensive host programs are executed. Our application mixes and the baseline configuration are summarized in Table \ref{tab:eval_config}. Overall, about 60\% of the internal-bus bandwidth is unused. However, the majority of idle periods are just $10-250$ cycles. Therefore, to utilize these idle periods for NDAs, mechanisms for fine-grain ownership switching is required. 

\begin{figure}[t!]
\centering
	\includegraphics[width=0.48\textwidth]{fig/motiv_rank_idle.pdf}
	\caption{Rank idle-time breakdown vs. idleness granularity.}
	\label{fig:motiv_rank_idle}
\end{figure}

% Need to add: "pre-charge all incurs high overhead --> need mechanisms with lowever overhead"

% NOTE: don't say that we are only targeting simple operations. Our approach can be applied to more complex operations as well, but poses more limitations. The opposite extreme of our approach is PEI, i.e. NDA per cacheline. 

\medskip
\noindent\textbf{\textit{How can the unique position of NDAs always sharing memory devices with the host be exploited?}}
% - Concurrent access on shared data without data reorganization
% - Fine-grain collaboration
% - Difficulties
%   - Data layout and address mapping
%   - Compelling use case
% - Make sure coherrence is not a problem here.
% - Just one copy of data

We focus on the uniqueness of NDAs compared to other discrete accelerators. If many different accelerators exist in a system, what will be the reasons to use NDAs? Unlike other accelerators, NDAs share high-capacity memory with the host and can access data with high peak bandwidth. This provides an opportunity of the host and NDAs to access the same data and collaboratively process them in fine-grain manner or even concurrently. The next question would be as follows: is there any application that can benefit from this collaboration enabled by the uniqueness of NDAs? Such application should meet the following requirements: (1) The application should be able to effectively leverage the specialties of each processor, (2) coherence should be handled infrequently, (3) both processors should work on large shared data. We introduce one use case, \textit{stochastic variance reduced gradient (SVRG)}, that satisfies these requirements, in Section \ref{sec:collaboration}.

% challenges
Since the host and NDAs share the same data, we cannot customize data layout for each processor. Prior work \cite{farmahini2015nda,akin2015hamlet} reorganizes data in between ownership switching but this approach cannot enable fine-grain access interleaving between the host and NDAs to the shared data. Therefore, the main challenge is on how to find an optimal single data layout. When either just the host or just the NDAs own memory for a fairly long time, we can customize data layout for each processor, possibly copying and laying out data differently when switching the memory ownership. However, concurrent NDA and host access to the same data requires a single data layout that works well for both the host and NDA at the same time. Otherwise, two copies of data with data layout are necessary, incurring high capacity overhead.

To meet the data-layout requirements of both processors, the following things should be considered. The host can maximally exploit bank-level parallelism when data is well-distributed across banks. To accomplish this, modern MCs use complex address hash function for physical-to-DRAM address mapping. On the other hand, NDAs can only fully utilize internal peak bandwidth when operands are all in local memory. 

\medskip
\noindent\textbf{\textit{How can we practically address the above questions under direct host control for non-packetized DRAMs?}}
% - Command bandwidth limitation
% - State synchronization
% - Bank partitioning
% - Memory allocation
 
To enable near-data acceleration and still benefit from deterministic and low memory latency of non-packetized DRAMs, the above problems should be resolved under direct host control. Though the host and NDAs seem to only share the internal DRAM bus, in fact, they contend for the command, address, and data (DAC) bus that connects between them since the host should control NDAs directly via the DAC bus. 

To mitigate this contention and realize high host and NDA performance, the following three problems should be resolved without frequent host-NDA communication. First, each memory controller should efficiently track global memory controller state for the fine-grain access interleaving. To track global memory controller state without always initializing it before the ownership switching, both MCs should frequently communicate each other. However, this method should be prevented to mitigate the contention on the DAC bus. 

Lastly, to minimize the number of NDA instructions launched by the host, each NDA instruction should include a lot of information in a compact format (which we call \textit{macro NDA instruction}) so that a few NDA instructions can make NDAs busy for a fairly long time. However, as addresses of operands are determined by the OS and host's memory controller, they should be calculated by the host and sent to NDAs for each cache block access of NDAs, such as PEI \cite{ahn2015pim}. Therefore, to enable macro NDA instructions, NDAs should figure out the address of next operands without host's help. 

\medskip
\noindent\textbf{\textit{Summary}}
To support host-NDA concurrent access to the same memory devices, the following problems should be resolved. 

\begin{itemize}[topsep=.5ex,itemsep=.5ex,partopsep=1ex,parsep=0ex]
	\item Fine-grain ownership switching is required to efficiently share the same memory among independent host and NDA processes.  
	\item A single data layout is required for the data shared between the host and NDAs to avoid capacity and performance overhead while collaboratively processing them.
	\item To solve the above problems under direct host control, the host and NDAs should minimally communicate while other necessary things, such as state tracking and instruction launching, are supported. 
\end{itemize}



 
 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

